HopPG: Self-Iterative Program Generation for Multi-Hop Question Answering over Heterogeneous Knowledge

The semantic parsing-based method is an important research branch for knowledge-based question answering. It usually generates executable programs lean upon the question and then conduct them to reason answers over a knowledge base. Benefit from this inherent mechanism, it has advantages in the performance and the interpretability. However, traditional semantic parsing methods usually generate a complete program before executing it, which struggles with multi-hop question answering over heterogeneous knowledge. On one hand, generating a complete multi-hop program relies on multiple heterogeneous supporting facts, and it is difficult for generators to understand these facts simultaneously. On the other hand, this way ignores the semantic information of the intermediate answers at each hop, which is beneficial for subsequent generation. To alleviate these challenges, we propose a self-iterative framework for multi-hop program generation (HopPG) over heterogeneous knowledge, which leverages the previous execution results to retrieve supporting facts and generate subsequent programs hop by hop. We evaluate our model on MMQA-T^2, and the experimental results show that HopPG outperforms existing semantic-parsing-based baselines, especially on the multi-hop questions.

==> experiment.tex <==
\section{Experiments}

\subsection{Dataset\label{dataset}}
The MMQA-T$^2$  used in this paper is a subset of MMQA \cite{2021MultiModalQA}. Specifically, we collect all questions based on tables and texts and exclude questions using images from MMQA, in a total of 15688 training instances and 1501 development instances.  Each question in MMQA is provided with 1 table together with 10 texts as candidate facts. The question type of the collect instances is shown in Table~\ref{questions}. Based on the question types, we re-split the training instances we collected in a ratio of 9:1 as the training set of the development set of  MMQA-T$^2$, respectively. The collected development instances from MMQA are directly used as the test set of  MMQA-T$^2$. We give the final basic statistics of MMQA-T$^2$ in Table~\ref{tab:dataset_sts}. 

To further demonstrate MMQA-T$^2$, we present the distribution of the training set questions in Table~\ref{questions} based on knowledge utilized, reasoning type, and the number of hops. It can be observed that 38.5\% of the questions are multi-hop, with 23.3\% of those requiring both tables and text to derive answers. These statistics indicate that MMQA-T$^2$ is a suitable dataset for evaluating HopPG, designed to improve question-answering performance in multi-hop reasoning over heterogeneous knowledge.


\begin{table*}[ht]
\centering
\small 
\begin{tabular}{c|c|c|c}
\hline
\textbf{Knowledge} & \textbf{Question Type} & \textbf{Hop}& \textbf{Distribution} \\
\hline
\multirow{6}{*}{Only Table}
& Cell / Multi-Cell &1& 42.5\%\\
& YesNo &1& 3.1\% \\
& Compose &2& 6.0\%\\
& Compare &2& 5.8\% \\
& Calculation &2& 0.6\% \\
& Intersect &2& 2.8\%\\
\hline
\multirow{2}{*}{Only Text}
& Span / Multi-span &1& 10.7\%\\
& YesNo &1& 5.1\%\\
\hline
\multirow{4}{*}{Table + Text} & Compose (table to text) &2& 9.4\%\\
 &Compose (text to table) &2& 4.8\%\\
 &YesNo (table to text) &2& 2.0\%\\
  &Intersect (table and text) &2& 4.1\%\\
  &Compare (Compose (text to the table)) &3& 3.0\%\\
\hline
\end{tabular}
% \setlength{\abovecaptionskip}{-0.000001cm}   
\caption{The question type distribution of the training set of MMQA-T$^2$.
}
\label{questions} 
\end{table*}
\begin{table*}[ht]
\centering
\small
\begin{tabular}{l|ccccccc|c}
\hline
Split &Span/Multi-span &Compare &Compose &YesNo & Calculation & Intersect & Compose\_Compare&Total\\
\hline
Train &7512&819&3463&1170&101&978&425&14122\\
Dev &834&90&346&130&11&108&47&1566\\
Test &748&70&383&142&6&88&64&1501\\
\hline
\end{tabular}
\caption{Basic statistics of MMQA-T$^2$.}\label{tab:dataset_sts}

\end{table*}


\subsection{Implementation Details}
The program generator of HopPG is initialized using BART-base and optimized with AdamW. The training settings are consistent with UniRPG. Specifically, the learning rate, batch size and weight decay are set to 1e-4, 128 and 0.01, respectively. When generating programs, we set the Beam Size of the beam search method as 4. The experiments are conducted on NVIDIA A100 GPU.
\subsection{Baselines}
\paragraph{AutoRouting and Implicit-Decomp}  These two baselines are from \cite{2021MultiModalQA}. We compare HopPG's question-answering performance with these baselines on the original MMQA dataset. For questions requiring images, we directly use the prediction results from Implicit-Decomp.
\paragraph{UniRPG} We reproduce the UniRPG-base version to directly generate complete multi-hop programs based on our operations. We select the top 2 candidate knowledge ranked by retrieval scores as the supporting facts. Then the question and the two facts are concatenated as input for UniRPG. In addition, we cut off the over-length input directly.
\subsection{Main Results}
Table~\ref{tab:mainres} shows the question-answering results of our HopPG and the baseline models. We use EM and F1 scores as the evaluation metrics and report the results on both the original MMQA and MMQA-T$^2$ datasets. For image-based questions in MMQA, we use the predictions of Implicit-Decomp. As the table shows, UniPRG, the first semantic parsing-based method on HQA tasks, achieves significant performance on MMQA-T$^2$ by 63.09 EM and 70.29 F1. It is proved that UniRPG can effectively solve the answer reasoning over tabular and textual knowledge by generating executable programs. 

Based on the results of UniRPG, our HopPG further brings improvements on MMQA-T$^2$. The EM scores increase by 1.37 on the single-hop questions and 1.22 on the multi-hop questions. The improvements are from the ability of HopPG to reduce the complexity of the supporting facts, and sufficiently utilize previous-hop execution results during program generations. These improvements demonstrate the effectiveness of HopPG. 

\subsection{Ablation Studies}
To provide a more detailed and intuitive demonstration of HopPG's performance on different question types, we compare the question-answering results between HopPG and baselines in Table~\ref{tab:abres}, where the results are reported on questions with different hop numbers and knowledge sources.

The results in the table indicate that Implicit-Decomp performs excellently on table-based questions, because it utilizes the table pre-trained model, TAPAS \cite{herzig-etal-2020-tapas}, for table-based question answering. Compared to TAPAS, semantic parsing-based models like UniRPG and HopPG offer the advantage of interpretability and avoid the need for expensive pre-training on a large number of tables. The table also shows that HopPG outperforms the baseline models on text-based questions because it generates programs using only the selected text as input, rather than simply concatenating complex and heterogeneous knowledge. This greatly reduces the difficulty of model inference.

As expected, HopPG achieves significant improvements in multi-hop question answering, which are mainly from the following three reasons: 1) Compared to directly generating complete programs, HopPG improves the accuracy of program generation at each hop by reducing the complexity of knowledge. 2) The program generation for each hop can refer to the execution results of the previous hop. 3) In HopPG, the errors in the program generated at the previous hop do not directly lead to incorrect results in the final output, which to some extent reduces error propagation.
%三跳问题还需要再解释一下
\begin{table*}[t]
\centering
\small

\begin{tabular}{l|ccc|ccc}
\hline
\textbf{Model} & \multicolumn{3}{c|}{MMQA} & \multicolumn{3}{c}{MMQA-T$^2$}\\
\hline
&\textbf{Overall}& \textbf{Single-hop}& \textbf{Multi-hop} &\textbf{Overall}& \textbf{Single-hop}& \textbf{Multi-hop}\\
\hline
AutoRouting &  42.10 / 49.05 & - & -&-&-&-\\
Implicit-Decomp  & 48.80 / 55.49& 51.61 / 58.36 & 44.59 /51.19 & 54.30 / 62.15 & 57.34 / 64.75 & 46.23 / 55.26\\

UniRPG$^{\dagger}$ & 53.87 / 60.20 & 57.22 / 64.05  & 48.87 / 54.45 & 63.09 / 70.29 & 65.05 / 72.72 & 56.69 / 63.84 \\
\hline
HopPG (ours) & \textbf{54.61} / \textbf{61.00} & 58.38 / 64.92 & 48.98 / 55.18 &\textbf{ 63.76} / \textbf{71.14} & 66.42 / 73.54 & 57.91 / 64.77  \\
\hline
\end{tabular}
% \setlength{\abovecaptionskip}{-0.000001cm}   
\caption{Results on the complete MMQA and the MMQA-T$^2$ datasets.}
\label{tab:mainres}

\end{table*}
\begin{table*}[t]
\centering
\small 
\begin{tabular}{c|c|c|c}
\hline
\textbf{Type} & \textbf{Implicit-Decomp} & \textbf{UniRPG$^{\dagger}$}& \textbf{MHPG} \\
\hline

TableQ &\textbf{72.35} / \textbf{79.89} & 63.41 / 69.93 & 65.04 / 70.33\\
TextQ &49.65 / 50.01& 65.60 / 73.64 & \textbf{67.13} / \textbf{75.19}  \\
Compose(TableQ,TextQ)  &50.00 / 56.70& 70.73 / 75.80& \textbf{71.95} / \textbf{75.99} \\
Compose(TextQ,TableQ)  &37.96 / 49.89 & 50.93 / 60.67 & \textbf{56.48} / \textbf{68.05}\\
Intersect(TableQ,TextQ) &48.98 / \textbf{55.24} & 44.89 / 48.63 & \textbf{48.98} / 54.24 \\
Compare(TableQ,Compose(TableQ,TextQ)) &\textbf{67.19} / \textbf{71.55}& 40.00 / 46.67 & 45.31 / 47.63\\

\hline
\end{tabular}
% \setlength{\abovecaptionskip}{-0.000001cm}   
\caption{The question type distribution of the training set of MMQA-T$^2$.
}
\label{tab:abres}
 
\end{table*}
%最好再加个case和error，
%case可以看看两跳问题里一跳错了但是2跳对了的例子，减少错误传播
%error中分析一下op错误和位置错误的比例，然后多条问题里两跳分别错误的比例，compose和intersect由于问题太像互相错分的比例

==> introduction.tex <==
\section{Introduction\label{intro}}
Question answering is a fundamental task and plays a crucial role in the field of natural language processing \cite{cui2020mutual,kwiatkowski2019natural,liu2020logiqa,choi2018quac,fan2019eli5}. In recent years, question-answering tasks based on heterogeneous knowledge (HQA) have increasingly gained the attention of researchers \cite{2020HybridQA,2020Open,2021TAT,2021MultiModalQA,2021FinQA}. These tasks require models to perform multi-hop reasoning on different structured knowledge, i.e., tables and texts. One category of the existing HQA method performs implicit answer reasoning, which takes the question and knowledge as input and performs reasoning in the semantic space, and then directly outputs the answer \cite{2020Unsupervised,2021Iterative,2022MuGER,2021MATE,2021Multi}. Although this approach has proven effective in HQA tasks, it lacks interpretability, scalability, and symbolic reasoning abilities. In contrast, the semantic parsing-based (SP-based)  approach explicitly derives answers by generating and executable programs, remedying the above-mentioned deficiencies and enabling researchers to monitor and improve each step of the derivation process.

SP-based methods have been widely used in question-answering tasks on homogeneous knowledge sources, such as tables, knowledge graphs, and texts \cite{yih2014semantic,bao2014knowledge,bao2016constraint,abdelaziz2021semantic,zhou2022opera}. Nevertheless, the SP-based question-answering methods over heterogeneous knowledge still require further exploration. Recently, \cite{zhou-etal-2022-unirpg} introduced UniRPG, the first SP-based model designed for HQA. 
%The authors employ the pre-trained transformer BART as the model's backbone and
They defined a set of general atomic and higher-order operations for discrete reasoning over heterogeneous knowledge resources. During the program generation process, UniRPG takes questions and supporting facts as input pairs of BART \cite{lewis-etal-2020-bart} to generate a complete program in a single step. Despite UniRPG's ability to generate programs using tables and passages with strict size limitations as oracles, its generation method is limited in open-domain multi-hop question-answering tasks.


Specifically, multi-hop reasoning usually requires multiple heterogeneous supporting facts, making it challenging for the model to retrieve and understand all the information simultaneously.
Additionally, these facts may exceed the length limitation of the model's input in terms of implementation. Moreover, generating a complete program sequence before executing can lead to a disconnect between the reasoning results of the current hop and the subsequent program generation. Intuitively, the reasoning results from the current hop are useful for selecting supporting facts and program generation in the next step. In addition, in this generation way, a generation error in any step will lead to an incorrect final answer. 
 
To tackle these issues, we introduce HopPG, an iterative program generation framework specifically designed for multi-hop answer reasoning based on heterogeneous knowledge. HopPG leverages the execution results of the previous program to select supporting facts and generate subsequent programs iteratively. In comparison to UniRPG, HopPG reduces the knowledge complexity used in each program generation step and incorporates information from the previous steps, enhancing the model's capability for multi-hop reasoning. Besides, in this generation way, the errors in the program generated at the previous hop do not directly lead to incorrect results in the final output, which reduces error propagation.

In this paper, we utilize a subset of the MMQA dataset \cite{2021MultiModalQA} for evaluating the effectiveness of HopPG. Specifically, we focus on questions based on tables and texts only, which we refer to as MMQA-T$^2$, excluding those requiring images as knowledge. Moreover, we construct a pseudo program for each question of MMQA-T$^2$ to enable weak supervision training. MMQA-T$^2$ was chosen as our dataset because it possesses the following notable characteristics: 1) questions are based on heterogeneous knowledge, 2) questions require multi-hop reasoning, and 3) MMQA-T$^2$ provides detailed annotations of the supporting facts and intermediate results for each hop, allowing us to construct more accurate pseudo programs. The experimental results show that HopPG outperforms existing semantic-parsing-based base-
lines, especially on the multi-hop questions.

Our contributions are summarized as follows: 
\begin{itemize}
    \item We propose HopPG, a self-iterative program generation framework designed for multi-hop question answering over heterogeneous knowledge. The framework successfully addresses the limitations of existing semantic parsing-based models. 
    \item We construct the MMQA-T$^2$ dataset based on MMQA, which only contains multi-hop questions over tabular and textual knowledge. Moreover, we construct pseudo-multi-hop programs for each question in MMQA-T$^2$ to train the program generator in a weak supervision way.
    \item We conduct extensive experiments and ablation studies on the MMQA-T$^2$ dataset. The experimental results show that HopPG outperforms the existing semantic-parsing-based QA model, especially on the multi-hop questions.
\end{itemize}

==> method.tex <==
\section{Methodology}
\subsection{Task Definition}
Multi-hop question answering over heterogeneous knowledge, i.e., tables and texts, aims to retrieve the supporting facts from the given knowledge and derive the answer to the question. 
Given a $H$-hop question $\mathcal{Q}$ and $K$ fact candidates $\mathcal{T}=\{t^1,...t^K\}$, the model requires deriving the final answer $a^H$ from $\mathcal{T}$. Apart from $a^H$, we use $\{a^1,...,a^{H-1}\}$ to represent the intermediate reasoning results in each hop. Each $a^h$, where $h \leq H$, can be a table cell, a text span, or a math calculation result.  The task is formalized as follows: 
\begin{align}
    a^H = \arg \max P(a^{H}|\mathcal{Q},\mathcal{T};\theta).
    \label{Eq:task}
\end{align}
 In this work, $\mathcal{T}$ contains a table and a set of texts. We assume that $t^1$ represents the table and the others $\{t^2,...,t^K\}$ are the $K$-$1$ texts. Specifically, the table $t^1$ consists of $m \times n$ cells $\{c_{ij}\}$, where $m$ and $n$ are the numbers of rows and columns. 


\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{fig/hoppg.png}
	\caption{The framework of  HopPG.}
	\label{model}
\end{figure*} 
\subsection{Model Overview}
To generate executable programs $\mathcal{P}$ to derive the answers over heterogeneous data, the existing model UniRPG \cite{zhou-etal-2022-unirpg} has defined a set of operations as reasoning units consisting of atomic and high-order operations.
We utilize and extend their operations in HopPG to allow for multi-hop reasoning and more reasoning types. 
Different  from UniRPG, which directly generates a complete program before executing, we decompose H-hop reasoning into multiple single hops, and the corresponding programs are defined as $\mathcal{P}$=$\{p^1,...,p^H\}$. Based on our program templates, HopPG generates the program $p^h$ hop by hop in an iterative way as Figure~\ref{model} shows. 

The figure also gives the framework of HopPG, which mainly contains three modules: fact retriever, program generator, and executor. The retriever and the generator are trainable and trained separately among these modules. During $h$-hop reasoning, the fact retriever first selects a supporting fact $t^h$ for the current hop based on the question $Q$ and the previous-hop result $a^{h-1}$. After that, the program generator receives $Q$, $a^{h-1}$ and $t^h$ as inputs and generate the program $p^h$. Subsequently, $p^h$ is executed by the program executor and $a^h$ can be derived. At this point, HopPG checks if the high-order operation of $p^h$ is a multi-hop operation\footnote{${\mathtt{COMPOSE}}$ and ${\mathtt{INTERSECT}}$, which are defined in Section~\ref{op}}. If it is, HopPG returns $a^h$ to iterate the above process. Otherwise, HopPG terminates the iteration and outputs $a^h$ as the final answer.


\subsection{Operations and Program Templates\label{op}}
\subsubsection{Multi-hop Operations}
\cite{zhou-etal-2022-unirpg} defined 15 operations for UniRPG, containing 4 atomic operations and 11 high-order operations. This work inherits a subset of their fundamental operations including ${\mathtt{CELL}}$,
${\mathtt{SPAN}}$,
${\mathtt{CELL\_VALUE}}$, ${\mathtt{SPAN\_VALUE}}$, ${\mathtt{KV}}$, ${\mathtt{MULTISPAN}}$, ${\mathtt{COUNT}}$, ${\mathtt{SUM}}$, ${\mathtt{AVG}}$, ${\mathtt{ARGMAX}}$, and ${\mathtt{ARGMIN}}$. Furthermore, we additionally extend multiple high-order operations to enable the programs to solve multi-hop questions and more reasoning types. The extended operations are listed as follows:
\begin{itemize}
    \item ${\mathtt{YESNO}}$: This is an atomic operation designed for "yes or no" reasoning. HopPG converts this reasoning type as a span extraction problem. Specifically, we connect two words, "Yes" and "No", with the question $Q$ as the input of the generator. The arguments of ${\mathtt{YESNO}}$ are the same as the other atomic operations, which are $(s, e)$. During execution, ${\mathtt{YESNO}}$ checks the extracted span, if it is "No", ${\mathtt{YESNO}}$ returns "No" as the answer. For all other cases, the operation returns "Yes". 
    
    \item ${\mathtt{COMPOSE}}$: This operation means the current hop is an intermediate hop, and the answering reasoning requires iteration. The argument of the ${\mathtt{COMPOSE}}$ is one of the atomic operations, ${\mathtt{CELL}}$ or ${\mathtt{SPAN}}$, and ${\mathtt{COMPOSE}}$ directly returns the result of the atomic operation as the current-hop result.
    
    \item ${\mathtt{INTERSECT}}$: This operation also means the current hop is an intermediate hop. Its argument is a high-order operation ${\mathtt{MULTISPAN}}$, and ${\mathtt{INTERSECT}}$ directly returns the results of   ${\mathtt{MULTISPAN}}$, a set of table cells or text spans.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\small
\centering
\begin{tabular}{c|c|c}
\hline
\multirow{2}{*}{\textbf{Reasoning Type} } &
\multicolumn{2}{c}{\textbf{Multi-hop Program Template}} \\\cline{2-3}
 &HOP-1 & HOP-2\\

\hline
\multirow{4}{*}{Span Extraction} 
& $\mathtt{CELL}$ $(s,e)$\\
& $\mathtt{CELL\_VALUE}$ $(s,e)$\\
& $\mathtt{SPAN}$ $(s,e)$\\
& $\mathtt{SPAN\_VALUE}$ $(s,e)$ \\
\hline
Multi-span Extraction & $\mathtt{MULTISPAN( CELL_1 / SPAN_1, ..., CELL_m / SPAN_m )}$ \\
\hline
YesNo &$\mathtt{YESNO}$ $(s,e)$\\
\hline
\multirow{2}{*}{Compare} 
& $\mathtt{ARGMAX (KV_1, KV_2)}$\\
& $\mathtt{ARGMIN (KV_1, KV_2)}$\\
\hline
Compose and Span Extraction & $\mathtt{COMPOSE(CELL / SPAN)}$ & $\mathtt{CELL / SPAN }$  \\
Compose and Multi-span Extraction & $\mathtt{COMPOSE(CELL / SPAN )}$ & $\mathtt{MULTISPAN}$\\
Compose and YesNo & $\mathtt{COMPOSE(CELL / SPAN}$ & $\mathtt{YESNO}$\\
\hline 
\multirow{4}{*}{Calculation}
& $\mathtt{SUM ( CV_{1}, ..., CV_{m} )}$\\
&$\mathtt{AVG ( CV_{1}, ..., CV_{m} )}$\\
& $\mathtt{COUNT ( CV_{1}, ..., CV_{m} )}$\\
\hline
Intersect	&$\mathtt{INTERSECT (MULTISPAN)}$ & $\mathtt{MULTISPAN}$\\
%hline
%Compose and Compare	& COMPARE(KV$_{1}$, KV ( HOP ( SPAN, CELL),CELL\_VALUE ) )\\

\hline
\end{tabular}
% \setlength{\abovecaptionskip}{-0.000001cm}   
\caption{The defined multi-hop program template for MMQA-T$^2$.
}
\label{temp}
 
\end{table*}
\subsubsection{Multi-hop Program Templates}
We define multi-hop program templates for questions of different reasoning types. These templates are used to construct pseudo programs for weakly supervised training and to constrain program generation.  We decompose the multi-hop reasoning into multiple single-hop programs. In this work, we set the maximum hop count\footnote{Very few (3\%) questions in the dataset need more than 2-hop reasoning.} $H$=2. The defined templates are listed in Table~\ref{temp}. Specifically, for questions of "compose" reasoning types, HopPG directly outputs the execution results of the 2-hop program as the final answer. In contrast, when tackling "intersect" questions, HopPG compares the results from the two hops and outputs the overlap cells or spans as the final answers. We execute the pseudo programs  constructed using our templates and evaluate the question-answering performance on the development set of MMQA-T$^2$, the EM and F1 scores are 91.27\% and 93.89\%, respectively.
\subsection{Supporting Fact Retriever}
The retriever in HopPG aims to select the supporting fact $t^h$ for the h-hop program generation  from the provided candidates, including a table and a set of texts. for the $h$-hop program generation. Following  \cite{yoran-etal-2022-turning}, we finetune the T5-3B \cite{2020t5} model using the training set of MMQA-T$^2$ as our retriever. The input of the retriever is a sequence consisting of the question $Q$, the golden execution result of the previous hop $a^{h-1}$, and one of the fact candidates $t^i$:
\begin{equation}
    \text{Inp}^{h}_{R}=[\langle s \rangle;Q;\langle \backslash s \rangle;a^{h-1};\langle \backslash s \rangle;t^i]
\end{equation}
Notably, the table $t^1$ is flattened by connecting its rows. For a first-hop example, the previous-hop execution result $a^0$ is set to "$\mathtt{None}$". The retriever receives the input sequences of all candidates and outputs a score vector $\bm \delta$=$(s^1,...,s^K)$ of them, then the model is fine-tuned using the following loss function, where $l$ is the golden fact's index:
\begin{equation}
{\mathcal{L^r}} = \mathtt{CrossEntropy}(l,\mathtt{Softmax}(\bm{ \delta}))
\end{equation}
After tuning, the supporting fact retrieval accuracy of our retriever is 90.7\%. During the program generation process, the tuned retriever ranks all candidate inputs and selects the fact $t^h$=$argmax(\bm \delta)$ as the supporting fact of the current hop $h$. 
\subsection{Program Generator}
The program generator aims to generate the corresponding program for each hop. In this work, we adopt UniRPG as the program generator of HopPG. It is a BART-based model equipped with a structure-aware knowledge reader \cite{zhang-etal-2020-table}, which is designed to enhance the table understanding ability of the encoder. We use the training set of MMQA-T$^2$ together with our constructed pseudo programs to train the UniRPG. 
Specifically, for  the $h$th-hop program generation, the input sequence consists of the question $Q$, the execution result of the previous-hop program $a^{h-1}$, and the supporting fact $t^h$ selected 
 by the retriever. We connect a text span \textit{"Yes or No"} to the question to transfer the $\mathtt{YESNO}$ reasoning type into a span extraction problem.
 Formally, the $h$th-hop input of our generator is represented as follows:
 \begin{equation}
    \text{Inp}^{h}_{G}=[\langle s \rangle;\text{Yes or No};Q;\langle \backslash s \rangle;a^{h-1};\langle \backslash s \rangle;t^h]
\end{equation}

The input sequence is fed into the structure-aware knowledge reader, which injects table structure information into the self-attention layers of the BART-encoder with structure-aware attention.
The reader learns the input and outputs the representations of input tokens:
Then, we feed it into the encoder to learn the representation $\mathbf{K} = \{\mathbf{k}_i\}_{i=1}^{L}$, where
L is the length of the input sequence.

Subsequently, the representations vectors $\mathbf{K}$ of the input tokens are used to decode the program based on our defined operations. The decoding process of HopPG is similar to UniRPG, with additional modifications to the operation vocabulary.  For the generator training, we gather the golden supporting facts and their corresponding programs for all hops of the questions. These data are utilized to train the program generator simultaneously.

\subsection{Program Executor}
To perform answer derivation, we implement a symbolic program executor for HopPG that executes the generated programs based on their meanings. When dealing with programs comprising multiple levels of operations, the executor executes from the atomic operations to the high-order operations.

\subsection{Iteration Detection}
In HopPG, we add an iteration detection process after the program execution to determine whether further hop generation and reasoning are needed. During the inference phase of HopPG, the iteration detection process checks the outermost operation of the current generated program to determine if it is one of the multi-hop operations, which include $\mathtt{COMPOSE}$ and $\mathtt{INTERSECT}$. If the operation belongs to multi-hop operations, HopPG performs the next hop generation iteratively. Otherwise, the current result is considered as the final answer.


==> related_work.tex <==
\section{Related Work}
\subsection{Question Answering over Heterogeneous Knowledge}
Previous works have attempted to leverage knowledge with various structures for question-answering, e.g., knowledge graphs and texts \cite{sun2019pullnet,han-etal-2020-open}. However, these researches are limited to using one type of knowledge as auxiliary information during answer reasoning and have not fully explored multi-hop reasoning across heterogeneous knowledge (HQA). To fill this gap, \cite{2020HybridQA} first propose the HybridQA task and dataset, which provides a WiKiTable  accompanied by hyperlinked Wikipedia passages as evidence for each question.
Based on HybridQA, \cite{chen2021ottqa} proposed the OTT-QA dataset, requiring the system to retrieve relevant tables and texts for their given question. Additionally, \cite{2021TAT} and \cite{2021FinQA} introduced TAT-QA and FinQA, both requiring numerical reasoning over heterogeneous data.

\subsection{Semantic Parsing-based Methods}
The semantic parsing-based methods reason answers by translating questions into executable programs such as SPARQL \cite{xiong2022autoqgs} and SQL\cite{hui-etal-2022-s2sql}. Previous semantic-parsing-based question-answering methods always research over homogeneous knowledge resources, i.e., texts \cite{zhou2022opera}, tables \cite{liu2022tapex} and knowledge graphs \cite{yih-etal-2016-value}. \cite{zhou-etal-2022-unirpg} proposed UniRPG, which first applies the semantic parsing-base method on question answering over heterogeneous knowledge including tables and texts. Based on their work, we propose HopPG in this paper to address the limitations of UniRPG in generating multi-hop programs based on heterogeneous knowledge.

